Diffusion Improves Graph Learning

Graph convolution is the core of most Graph Neural Networks (GNNs) and usually approximated by message passing between direct (one-hop) neighbors. In this work, we remove the restriction of using only the direct neighbors by introducing a powerful, yet spatially localized graph convolution: Graph diffusion convolution (GDC). GDC leverages generalized graph diffusion, examples of which are the heat kernel and personalized PageRank. It alleviates the problem of noisy and often arbitrarily defined edges in real graphs. We show that GDC is closely related to spectral-based models and thus combines the strengths of both spatial (message passing) and spectral methods. We demonstrate that replacing message passing with graph diffusion convolution consistently leads to significant performance improvements across a wide range of models on both supervised and unsupervised tasks and a variety of datasets. Furthermore, GDC is not limited to GNNs but can trivially be combined with any graph-based model or algorithm (e.g. spectral clustering) without requiring any changes to the latter or affecting its computational complexity. Our implementation is available online.

==> tables/hyper_citeseer.tex <==

    \begin{table}[h]
        \centering
        \caption{Hyperparameters for \textsc{Citeseer}.}
        \label{tab:hyper:citeseer}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{llrllrlrrr}

Model & Diffusion &  $\alpha$ & $t$ &  $k$ &  $\epsilon$ & Architecture &  $\lambda_{\text{L2}}$ &  Learning rate &  Dropout \\
\hline
\multirow{4}{*}{GCN} & - &         - &   - &    - &           - &         1x64 &                 0.0593 &           0.01 &      0.5 \\
     & Heat &         - &   5 &    - &      0.0001 &         1x64 &                 0.0861 &           0.01 &      0.5 \\
     & PPR &      0.15 &   - &  128 &           - &         1x64 &                 0.0960 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &  128 &           - &         1x64 &                 0.0814 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{GAT} & - &         - &   - &    - &           - &       1x2x64 &                 0.0593 &           0.01 &      0.5 \\
     & Heat &         - &   1 &    - &      0.0010 &       1x2x64 &                 0.0826 &           0.01 &      0.5 \\
     & PPR &      0.10 &   - &    - &      0.0005 &       1x2x64 &                 0.0964 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &    - &      0.0005 &       1x2x64 &                 0.0408 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{JK} & - &         - &   - &    - &           - &         4x64 &                 0.0593 &           0.01 &      0.5 \\
     & Heat &         - &   5 &    - &      0.0001 &         2x64 &                 0.0861 &           0.01 &      0.5 \\
     & PPR &      0.15 &   - &  128 &           - &         2x64 &                 0.0960 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &  128 &           - &         2x64 &                 0.0814 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{GIN} & - &         - &   - &    - &           - &         5x64 &                 0.0676 &           0.01 &      0.5 \\
     & Heat &         - &   5 &    - &      0.0005 &         5x64 &                 0.0854 &           0.01 &      0.5 \\
     & PPR &      0.10 &   - &  128 &           - &         5x64 &                 0.0141 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &  128 &           - &         5x64 &                 0.0487 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{ARMA} & - &         - &   - &    - &           - &       3x1x16 &                 0.0830 &           0.01 &      0.5 \\
     & Heat &         - &   5 &   64 &           - &       3x1x16 &                 0.0816 &           0.01 &      0.5 \\
     & PPR &      0.15 &   - &  128 &           - &       3x1x16 &                 0.0824 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &  128 &           - &       3x1x16 &                 0.0938 &           0.01 &      0.5 \\

\end{tabular}
        }
    \end{table}

==> tables/hyper_coauthorcs.tex <==

    \begin{table}[h]
        \centering
        \caption{Hyperparameters for \textsc{Coauthor CS}.}
        \label{tab:hyper:coauthorcs}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{llrllrlrrr}

Model & Diffusion &  $\alpha$ & $t$ &  $k$ &  $\epsilon$ & Architecture &  $\lambda_{\text{L2}}$ &  Learning rate &  Dropout \\
\hline
\multirow{4}{*}{GCN} & - &         - &   - &   - &           - &         1x64 &                 0.0570 &           0.01 &      0.5 \\
     & Heat &         - &   1 &  64 &           - &         1x64 &                 0.0806 &           0.01 &      0.5 \\
     & PPR &       0.1 &   - &  64 &           - &         1x64 &                 0.0313 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &  64 &           - &         1x64 &                 0.0302 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{GAT} & - &         - &   - &   - &           - &       2x2x64 &                 0.0039 &           0.01 &      0.5 \\
     & Heat &         - &   1 &   - &      0.0005 &       1x2x64 &                 0.0256 &           0.01 &      0.5 \\
     & PPR &       0.1 &   - &   - &      0.0005 &       1x2x64 &                 0.0043 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &  64 &           - &       1x2x64 &                 0.0164 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{JK} & - &         - &   - &   - &           - &         2x64 &                 0.0227 &           0.01 &      0.5 \\
     & Heat &         - &   1 &  64 &           - &         2x64 &                 0.0264 &           0.01 &      0.5 \\
     & PPR &       0.1 &   - &  64 &           - &         2x64 &                 0.0313 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &  64 &           - &         2x64 &                 0.0164 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{ARMA} & - &         - &   - &   - &           - &       2x1x16 &                 0.0161 &           0.01 &      0.5 \\
     & Heat &         - &   1 &  64 &           - &       3x1x16 &                 0.0105 &           0.01 &      0.5 \\
     & PPR &       0.1 &   - &  64 &           - &       2x1x16 &                 0.0141 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &  64 &           - &       2x1x16 &                 0.0343 &           0.01 &      0.5 \\

\end{tabular}
        }
    \end{table}

==> tables/hyper_computers.tex <==

    \begin{table}[h]
        \centering
        \caption{Hyperparameters for \textsc{Amz Comp}.}
        \label{tab:hyper:computers}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{llrllrlrrr}

Model & Diffusion &  $\alpha$ & $t$ &  $k$ &  $\epsilon$ & Architecture &  $\lambda_{\text{L2}}$ &  Learning rate &  Dropout \\
\hline
\multirow{4}{*}{GCN} & - &         - &   - &    - &           - &         1x64 &                 0.0278 &           0.01 &      0.5 \\
     & Heat &         - &   5 &    - &      0.0010 &         1x64 &                 0.0682 &           0.01 &      0.5 \\
     & PPR &       0.1 &   - &   64 &           - &         1x64 &                 0.0401 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &   64 &           - &         1x64 &                 0.0164 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{GAT} & - &         - &   - &    - &           - &       1x2x64 &                 0.0934 &           0.01 &      0.5 \\
     & Heat &         - &   1 &    - &      0.0005 &       1x2x64 &                 0.0101 &           0.01 &      0.5 \\
     & PPR &       0.1 &   - &    - &      0.0005 &       1x2x64 &                 0.0298 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &   64 &           - &       1x2x64 &                 0.0164 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{JK} & - &         - &   - &    - &           - &         2x64 &                 0.0278 &           0.01 &      0.5 \\
     & Heat &         - &   5 &    - &      0.0010 &         2x64 &                 0.0682 &           0.01 &      0.5 \\
     & PPR &       0.1 &   - &   64 &           - &         2x64 &                 0.0394 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &   64 &           - &         2x64 &                 0.0302 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{GIN} & - &         - &   - &    - &           - &         6x64 &                 0.0121 &           0.01 &      0.5 \\
     & Heat &         - &   3 &   64 &           - &         5x64 &                 0.0023 &           0.01 &      0.5 \\
     & PPR &       0.1 &   - &   64 &           - &         5x64 &                 0.0373 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &   64 &           - &         5x64 &                 0.0224 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{ARMA} & - &         - &   - &    - &           - &       3x1x16 &                 0.0060 &           0.01 &      0.5 \\
     & Heat &         - &   5 &   64 &           - &       3x1x16 &                 0.0350 &           0.01 &      0.5 \\
     & PPR &       0.1 &   - &  128 &           - &       2x1x32 &                 0.0631 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &   64 &           - &       3x1x16 &                 0.0057 &           0.01 &      0.5 \\

\end{tabular}
        }
    \end{table}

==> tables/hyper_cora.tex <==

    \begin{table}[h]
        \centering
        \caption{Hyperparameters for \textsc{Cora}.}
        \label{tab:hyper:cora}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{llrllrlrrr}

Model & Diffusion &  $\alpha$ & $t$ &  $k$ &  $\epsilon$ & Architecture &  $\lambda_{\text{L2}}$ &  Learning rate &  Dropout \\
\hline
\multirow{4}{*}{GCN} & - &         - &   - &    - &           - &         1x64 &                 0.0593 &           0.01 &      0.5 \\
     & Heat &         - &   5 &    - &      0.0001 &         1x64 &                 0.0861 &           0.01 &      0.5 \\
     & PPR &      0.05 &   - &  128 &           - &         1x64 &                 0.0960 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &  128 &           - &         1x64 &                 0.0814 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{GAT} & - &         - &   - &    - &           - &       1x2x64 &                 0.0593 &           0.01 &      0.5 \\
     & Heat &         - &   1 &    - &      0.0010 &       1x2x64 &                 0.0357 &           0.01 &      0.5 \\
     & PPR &      0.10 &   - &    - &      0.0050 &       1x2x64 &                 0.0788 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &    - &      0.0010 &       1x2x64 &                 0.0408 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{JK} & - &         - &   - &    - &           - &         3x64 &                 0.0410 &           0.01 &      0.5 \\
     & Heat &         - &   5 &    - &      0.0001 &         2x64 &                 0.0861 &           0.01 &      0.5 \\
     & PPR &      0.05 &   - &  128 &           - &         2x64 &                 0.0960 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &  128 &           - &         2x64 &                 0.0487 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{GIN} & - &         - &   - &    - &           - &         5x64 &                 0.0858 &           0.01 &      0.5 \\
     & Heat &         - &   3 &    - &      0.0001 &         6x64 &                 0.0724 &           0.01 &      0.5 \\
     & PPR &      0.05 &   - &  128 &           - &         5x64 &                 0.0141 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &  128 &           - &         4x64 &                 0.0244 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{ARMA} & - &         - &   - &    - &           - &       3x1x16 &                 0.0412 &           0.01 &      0.5 \\
     & Heat &         - &   5 &   64 &           - &       2x1x16 &                 0.0816 &           0.01 &      0.5 \\
     & PPR &      0.10 &   - &  128 &           - &       3x1x16 &                 0.0462 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &  128 &           - &       2x1x16 &                 0.0503 &           0.01 &      0.5 \\

\end{tabular}
        }
    \end{table}

==> tables/hyper_photo.tex <==

    \begin{table}[h]
        \centering
        \caption{Hyperparameters for \textsc{Amz Photo}.}
        \label{tab:hyper:photo}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{llrllrlrrr}

Model & Diffusion &  $\alpha$ & $t$ &  $k$ &  $\epsilon$ & Architecture &  $\lambda_{\text{L2}}$ &  Learning rate &  Dropout \\
\hline
\multirow{4}{*}{GCN} & - &         - &   - &    - &           - &         1x64 &                 0.0278 &           0.01 &      0.5 \\
     & Heat &         - &   3 &    - &      0.0001 &         2x64 &                 0.0816 &           0.01 &      0.5 \\
     & PPR &      0.15 &   - &   64 &           - &         1x64 &                 0.0324 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &   64 &           - &         1x64 &                 0.0164 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{GAT} & - &         - &   - &    - &           - &       1x2x64 &                 0.0767 &           0.01 &      0.5 \\
     & Heat &         - &   1 &    - &      0.0005 &       1x2x64 &                 0.0101 &           0.01 &      0.5 \\
     & PPR &      0.10 &   - &    - &      0.0005 &       2x2x64 &                 0.0668 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &   64 &           - &       1x2x64 &                 0.0164 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{JK} & - &         - &   - &    - &           - &         2x64 &                 0.0278 &           0.01 &      0.5 \\
     & Heat &         - &   3 &    - &      0.0005 &         2x64 &                 0.0682 &           0.01 &      0.5 \\
     & PPR &      0.15 &   - &   64 &           - &         2x64 &                 0.0299 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &   64 &           - &         2x64 &                 0.0164 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{GIN} & - &         - &   - &    - &           - &         5x64 &                 0.0137 &           0.01 &      0.5 \\
     & Heat &         - &   3 &   64 &           - &         5x64 &                 0.0023 &           0.01 &      0.5 \\
     & PPR &      0.10 &   - &   64 &           - &         5x64 &                 0.0373 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &   64 &           - &         5x64 &                 0.0224 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{ARMA} & - &         - &   - &    - &           - &       3x1x16 &                 0.0060 &           0.01 &      0.5 \\
     & Heat &         - &   3 &   64 &           - &       2x1x16 &                 0.0350 &           0.01 &      0.5 \\
     & PPR &      0.15 &   - &  128 &           - &       2x1x32 &                 0.0631 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &   64 &           - &       2x1x16 &                 0.0057 &           0.01 &      0.5 \\

\end{tabular}
        }
    \end{table}

==> tables/hyper_pubmed.tex <==

    \begin{table}[h]
        \centering
        \caption{Hyperparameters for \textsc{PubMed}.}
        \label{tab:hyper:pubmed}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{llrllrlrrr}

Model & Diffusion &  $\alpha$ & $t$ &  $k$ &  $\epsilon$ & Architecture &  $\lambda_{\text{L2}}$ &  Learning rate &  Dropout \\
\hline
\multirow{4}{*}{GCN} & - &         - &   - &    - &           - &         1x64 &                 0.0257 &           0.01 &      0.5 \\
     & Heat &         - &   3 &    - &      0.0001 &         1x64 &                 0.0420 &           0.01 &      0.5 \\
     & PPR &       0.1 &   - &   64 &           - &         1x64 &                 0.0561 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &  128 &           - &         2x64 &                 0.0146 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{GAT} & - &         - &   - &    - &           - &       2x2x64 &                 0.0257 &           0.01 &      0.5 \\
     & Heat &         - &   1 &    - &      0.0005 &       2x2x64 &                 0.0162 &           0.01 &      0.5 \\
     & PPR &       0.1 &   - &    - &      0.0005 &       2x2x64 &                 0.0027 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &  128 &           - &       2x2x64 &                 0.0146 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{JK} & - &         - &   - &    - &           - &         2x64 &                 0.0532 &           0.01 &      0.5 \\
     & Heat &         - &   3 &    - &      0.0001 &         2x64 &                 0.0883 &           0.01 &      0.5 \\
     & PPR &       0.1 &   - &   64 &           - &         2x64 &                 0.0250 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &  128 &           - &         3x64 &                 0.0146 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{GIN} & - &         - &   - &    - &           - &         5x64 &                 0.0756 &           0.01 &      0.5 \\
     & Heat &         - &   3 &    - &      0.0010 &         6x64 &                 0.0191 &           0.01 &      0.5 \\
     & PPR &       0.1 &   - &   64 &           - &         6x64 &                 0.0149 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &   64 &           - &         6x64 &                 0.0255 &           0.01 &      0.5 \\
\cline{1-10}
\multirow{4}{*}{ARMA} & - &         - &   - &    - &           - &       2x1x16 &                 0.0040 &           0.01 &      0.5 \\
     & Heat &         - &   3 &    - &      0.0001 &       2x1x16 &                 0.0016 &           0.01 &      0.5 \\
     & PPR &       0.1 &   - &   64 &           - &       3x1x16 &                 0.0051 &           0.01 &      0.5 \\
     & AdaDIF &         - &   - &   64 &           - &       2x1x16 &                 0.0057 &           0.01 &      0.5 \\

\end{tabular}
        }
    \end{table}
